Integral mixed motives in equal characteristic

For noetherian schemes of finite dimension over a field of characteristic exponent $p$, we study the triangulated categories of $\mathbf{Z}[1/p]$-linear mixed motives obtained from cdh-sheaves with transfers. We prove that these have many of the expected properties. In particular, the formalism of the six operations holds in this context. When we restrict ourselves to regular schemes, we also prove that these categories of motives are equivalent to the more classical triangulated categories of mixed motives constructed in terms of Nisnevich sheaves with transfers. Such a program is achieved by comparing these various triangulated categories of motives with modules over motivic Eilenberg-MacLane spectra.

==> HZmod.tex <==
\subsection{Modules over motivic cohomology} The idea of considering modules
 over the spectrum representing motivic cohomology is a natural one, in view
 of \cite{OR}. We explain this construction in this paragraph, using the
 (stable) $\AA^1$-derived category of Morel $\Der_{\AA^1}(-,R)$.

\begin{paragr}
The motivic triangulated category $\Der_{\AA^1}(-,R)$ is constructed
 using the usual step of $\AA^1$-localization and $\PP^1$-stabilization
 from the premotivic abelian category of Nisnevich sheaves of $R$-modules
 over the smooth-Nisnevich site: $\sh(-,R)$.

The link with motives in this setting is very easy as there exists
 a premotivic adjunction:
\begin{equation} \label{eq:premotivic_adj_transfers}
\gamma^*:\sh(-,R) \rightleftarrows \shtr(-,R):\gamma_*
\end{equation}
where the functor $\gamma_*$ simply forgets transfers. 
Applying the $\AA^1$-localization and $\PP^1$-stabilization
 process to the derived cattegories, we get an adjunction
of premotivic triangulated categories:
$$
\derL \gamma^*:\Der_{\AA^1}(S,R) \rightleftarrows \DM(S,R):\derR \gamma_*.
$$
It formally follows that the object $\derR \gamma_*(\un_S)$ is a commutative 
 ring spectrum which represents motivic cohomology in $\Der_{\AA^1}(S,R)$.
 Let us consider the adjunction of premotivic model categories
 underlying the preceding one and induced by \eqref{eq:premotivic_adj_transfers}
 on the level of $\PP^1$-spectra:
$$
\gamma^*:\Sp(S,R) \rightleftarrows \Sp^{tr}(S,R):\gamma_*.
$$
The functor $\gamma_*$ preserves stable $\AA^1$-equivalences so that
 $\derR \gamma_*=\gamma_*$. It follows that if we apply the symmetric
 spectrum $\HZ_S=\gamma_*(\un_S)$ is a strict (commutative) ring spectrum representing 
 motivic cohomology. By construction, this objets agree with
 (the $R$-linearisation of) the one defined by Voevodsky in \cite[Sec. 6.1]{V3}.

The major issue with this construction is that, given a morphism
 of schemes $f:T \rightarrow S$, the canonical map:
$$
\tau_f:\derL f^*(\HZ_S) \rightarrow \HZ_T
$$
is not necessarily an isomorphism in $\Der_{\AA^1}(T,R)$
 though if it is obviously true when $f$ is smooth --
 because then, according to the basic properties of a
 premotivic adjunction, $\derL f^* \gamma_*=\gamma_* \derL f^*$
 (see also \ref{conjecture_pullback} for further results).
\end{paragr}


==> tstructure.tex <==
\begin{num}
The perverse homotopy $t$-structure
 was introduced by Ayoub in \cite{ayoub}.
 More precisely, he studied after Morel
 $t$-structure which satisfies the gluing formalism
 on stable homotopy functors.

Let us recall the definition of this $t$-structure.
 According to \cite{ayoub}, it is possible
 to describe $t$-structures on a compactly generated
 triangulated category\footnote{\emph{i.e.} a triangulated
 category which admits small sums and such 
 that there exists a set of generators which are compact.}
 $\T$ as follows.

First, given a set of compact objects $\mathcal G$ in $\T$,
 we let $\langle \langle \mathcal G \rangle \rangle_+$ be
 the smallest full subcategory $\T_0$ of $\T$ such that:
\begin{itemize}
\item for any $A \in \mathcal G$, $A$ is an object of $\T_0$;
\item given any distinguished triangle in $T$,
$$
A' \rightarrow A \rightarrow A'' \rightarrow A'[1]
$$
if $A'$ and $A''$ belongs to $\T_0$, then $A$ belongs to $\T_0$;
\item $\T_0$ is closed under small sums;
\item $\T_0$ is closed under suspension: $A$ belongs to $\T_0$
 implies $A[1]$ belongs to $\T_0$.
\end{itemize}

Then Ayoub  proved the following result
 (see \cite[2.1.70]{ayoub}) which he attributes to Morel:
\end{num}
\begin{prop}
Consider the above assumptions and put:

$\T_{\geq 0}=\langle \langle \mathcal G \rangle \rangle_+$,
 $\T_{<0}=(\T_{\geq 0})^{\perp}$.\footnote{As usual,
 given a full subcategory $\mathcal U$ of $\T$,
 we denote by $\mathcal U^{\perp}$
 the full additive subcategory consisting of the objects $B \in \T$
 satisfying $\Hom_\T(A,B)=0$ for all $A \in \mathcal U$.} \\
Then the pair $(\T_{\geq 0},\T_{<0})$ defines a $t$-structure on $\T$.
\end{prop}
In the assumptions of the proposition,
 the pair $(\T_{\geq 0},\T_{<0})$ is called the \emph{$t$-structure generated
 by $\mathcal G$.}

\begin{rem}
This result is best described using the notion of \emph{aisle}
 introduced in \cite[\textsection 1]{KelVoi}: it can be
 restated by saying that the inclusion functor
$$
\langle \langle \mathcal G \rangle \rangle_+ \rightarrow \T
$$
admits a right adjoint.
Acording to this remark, we can relax the assumption that
 $\T$ is compactly generated. For example, if $\T$
 is the homotopy category of a left proper combinatorial
 model category, the theory of Bousfield localization
 provides the right adjoint for any set of objects $\mathcal G$.
The same is true using results of Lurie if $\T$
 is the homotopy category of a presentable stable $\infty$-category.
Finally that one should be able to replace 
 compactly generated by well generated in the sense of Neeman
 but we do not know any reference. 
\end{rem}

The following definition is essentially due to Morel:
\begin{df}
Let $\T$ be a premotivic triangulated category
 which is compactly generated by Tate twists
 (cf \cite[1.3.16]{CD3}).\footnote{\emph{i.e.} given any $k$-scheme $S$,
 $\T(S)$ is generated by objects $M_S(X)(n)$ for
 $X/S$ smooth and $n \in \ZZ$, and these objects
 are compact.}

Given any $k$-scheme $S$,
 we define the \emph{homotopy $t$-structure} on $\T(S)$
 as the $t$-structure generated by the following objects:
$$
M_S(X)(n)[n]
$$
for a smooth scheme $X/S$ and an integer $n \in \ZZ$.

We denote simply by $t$ this $t$-structure. 
\end{df}

\begin{ex}\label{ex:htp&perverse-htp}
The homotopy $t$-structure on $\DM(k)$ coincides
 with Voevodsky's homotopy $t$-structure (see \cite{Deg8}).
 The homotopy $t$-structure on $\SH(k)$ coincides
 with Morel's homotopy $t$-structure (see \cite[Rem. 1.1.5]{Deg10}).
\end{ex}

\begin{num}
We will need a finer $t$-structure defined by Ayoub.
We will define it on any 
We will define it within a motivic triangulated
 category $\T$ over $k$-schemes which is generated by Tate twists.

Recall this assumption guarantees that 
 a $\T$-motives over $S$ is constructible if and only if it
 is compact (see \cite[1.4.11]{CD3}).
 Let $\T_c(S)$ be the full subcategory made by constructible
 $\T$-motives over $S$.
According to \cite[2.2.37]{ayoub},
 we get that $\T_c(S)$ is stable under the 6 operations
 (here we use that $k$ is of characteristic $0$).
\end{num}
\begin{df}
Let  $\T$ be a motivic triangulated category
 satisfying the above assumptions.

Given any separated $k$-scheme $S$ of finite type,
 we define the \emph{perverse homotopy $t$-structure on $\T(S)$}
 as the $t$-structure generated by the following objects:
$$
f_!p^!(\un_k)(n)[n]
$$
where $f:X \rightarrow S$ is a $k$-morphism 
 for a separated $k$-scheme of finite type $X$,
 $p$ is the structural morphism of $X/k$,
 and $n \in \ZZ$ is any integer.

We denote by $t^p$ this $t$-structure
 and by $\pheart\T(S)$ its heart.
\end{df}

\begin{rem}
Let $f:Y \rightarrow X$ be a separated morphism of finite type 
 between $k$-schemes of finite type.

Then, it is obvious that $f_!$ preserves the generators
 of the $t^p$-positive objects.
 Thus, $f^!$ (resp. $f^!$) is $t^p$-positive
 (resp. $t^p$-negative).

When moreover $f^!$ is smooth,
it follows from relative purity and the base change theorem
 that $f^!$ preserves the generators
 of the $t^p$-positive objects. Thus, $f^!$ is $t^p$-exact.
\end{rem}


\begin{ex} \label{ex:p-htp_field}
According to \cite[2.2.86, 2.2.82]{ayoub},
 the homotopy and perverse homotopy $t$-structures
 on $\T(k)$ coincides
 (here we use that $k$ is of characteristic $0$,
 but see Remark \ref{rem:generalization_htptstr}
 in the case of positive characteristic).
 The same is true for $\T(E)$ here $E/k$
 is any finite field extension.
\end{ex}

We will need the following proposition due to Ayoub:
\begin{prop} \label{prop:basic_tp-exactness}
Let $\T$ be as in the above definition.

Let $i:Z \rightarrow S$ be a closed immersion
 with complementary open immersion $j:U \rightarrow S$.
 Then the following assertions hold:
\begin{enumerate}
\item $i^*$ is $t^p$-positive and $i_*$ is $t^p$-exact;
\item $j_!$ is $t^p$-positive and $j^*$ is $t^p$-exact;
\item a $\T$-motive $M$ is $t^p$-positive if and only
 if $j^*(M)$ and $i^*(M)$ are so.
\end{enumerate}
\end{prop}
\begin{proof}
Note that Point (2) follows from the preceding remark.
Then, refering to \emph{loc. cit.},
 Point (1) is proved in 2.2.77 and 2.2.78
 and Point (3) is a formal consequence
 of (1)+(2) and the localization property of $\T$.
\end{proof}


\begin{rem}\label{rem:generalization_htptstr}
In fact, to prove that the preceding Proposition is true,
 according to the proof of the results mentioned above,
 we only need to prove Proposition 2.2.69 of \emph{loc. cit.}
 which amounts to the following assumption on $\T$
 (as we work over a perfect field $k$):
\begin{itemize}
\item Then for any separated $k$-scheme $S$ of finite type,
 and any closed subscheme $Z \subset S$,
 the perverse homotopy $t$-structure over $S$ is generated
 by the objects of the form:
$$
f_!p^!(\un_k)(n)[n]
$$
where $f:X \rightarrow S$ is a projective morphism 
 with $X$ a regular $k$-scheme with structural morphism $p$
 and $f^{-1}(Z)$ is either equal to $X$ of the support
 of a normal crossing divisor.
\end{itemize}
Indeed, this assumption formally implies:
\begin{enumerate}
\item given any separated morphism of finite type $f:X \rightarrow S$,
 the functor $f^!$ is $t^p$-exact: this is \emph{loc. cit.} 2.2.72 (see its proof).
\item given any open immersion $j$ with complementary closed immersion $i$,
 the functor $j_*$ is $t^p$-exact and the functor $i^*j_*[-1]$ is
  $t^p$-positive: this is \emph{loc. cit.} 2.2.75.
\item same notations as in (2): the functor $i^*$ is $t^p$-positive:
 this follows from point (1) and (2) above, according to
 the localization triangle:  this is \emph{loc. cit.} 2.2.77.
\item same notations as in (2): the functor $i_*$ is $t^p$-exact:
 this follows from point (3) above, and the fact $i_*$ is obviously
 $t^p$-positive:  this is \emph{loc. cit.} 2.2.78.  
\end{enumerate}

Note that to get the result of Example \ref{ex:htp&perverse-htp},
 we need the above assumption and the assumption that
 $\T$ is \emph{semi-separated}.
This is used both in \emph{loc. cit.} 2.2.82 and 2.2.86
 -- note the semi-separatedness assumption
  does not appear in the statement of 2.2.86 but it is
	used in the proof as it appeal to 2.2.55 which needs
	this assumption.

Unfortunately, the separatedness assumption is not known for
 $\SH[1/p]$ or $\DMt[1/p]$, so we cannot extend Theorem 
 \ref{thm:heart&eta} below
 to the case of fields of positive characteristic,
 even after inverting $p$.
\end{rem}


We formally deduce from that theorem the following corollary:
\begin{cor}\label{cor:tp-glueing}
Using the notations of the previous corollary,
 the abelian category $\pheart\T(S)$ is the glueing of the
 abelian categories $\pheart\T(Z)$ and $\pheart\T(U)$ along
 the following exact functors:
$$
\pheart\T(Z) \xrightarrow{i_*} \pheart\T(X)
 \xrightarrow{j^*}  \pheart\T(U).
$$
Moreover, the left (resp. right) adjoint functor
 to $i_*$ is $\ptau^p_{\leq 0}(i^*)$ (resp. $\ptau^p_{\geq 0}(i^*)$)
 and the left (resp. right) adjoint functor tp $j^*$
 is $\ptau^p_{\leq 0}(j_!)$ (resp. $\ptau^p_{\geq 0}(j_*)$).
\end{cor}

The following result is obtain using the same proof
 as \cite[4.4.25]{CD3} but using Hironaka resolution
 of singularities as we have restricted to characteristic
 $0$:
\begin{prop}
Let $\varphi^*:\T \leftrightarrows \T':\varphi_*$
 be an adjunction of motivic triangulated categories
 over $k$-schemes of finite type.
 Assume $\T$ and $\T'$ are generated by Tate twists.

Then the induced functor $\varphi^*:\T_c \rightarrow \T'_c$
 between the constructible parts
 commutes with the 6 operations.
\end{prop}

\begin{cor}
Consider the assumptions of the previous
 proposition and assume $\T$, $\T'$ are compactly
 generated by their Tate twist.

Then $\varphi^*$ (resp. $\varphi_*$) is
 $t^p$-positive (resp. $t^p$-negative).
\end{cor}
Indeed, according to the previous
 proposition, $\varphi^*$ preserves
 the generators of the perverse $t$-structure.
 The assertion for $\varphi_*$ is a formal consequence.

\begin{num}
We will consider the following adjuntions of motivic
 triangulated categories:
$$
\xymatrix@=30pt{
\SH\ar@<2pt>^-K[r] & \DMt\ar@<2pt>^-{\gamma^*}[r]\ar@<2pt>^-N[l]
 & \DMcdh\ar@<2pt>^-{\gamma_*}[l]
}
$$
where $(K,N)$ is induced by the Dold-Kan equivalence
 (see \cite[\textsection 4]{ayoub2})
 and $(\gamma^*,\gamma_*)$ if induced by the functor
 adding transfers at the level of sheaves.

According to its construction, the functor $N$ commutes with
 $j_\sharp$ for $j$ an open immersion.
 The same is true for $\gamma_*$ according to \cite[6.3.11]{CD3}
  (more precisely its variant for the $\cdh$-topology). We easily
	 deduce our first lemma:
\end{num}
\begin{lm}
The functors $N$ and $\gamma_*$ above
 are $t^p$-exact.
\end{lm}
\begin{proof}
Indeed, these two functors formally commutes with
 $f_*$ and $p^!$ (see \cite[2.4.53]{CD3}).
According to the construction of $p_!$ in \cite{CD3}
 and the remark preceding the lemma, they also commutes
 with $p_!$. Thus they preserve the generators
 of the perverse homotopy $t$-structure, so they are
 $t^p$-positive. The preceding corollary allows to conclude.
\end{proof}

\begin{num}\label{num:wk_orientable}
Following the terminology of \cite{Deg10},
 we will say that a spectrum $\mathbb E$ in $\SH(S)$
 is \emph{weakly orientable} if $\eta \wedge \mathbb E=0$
 where $\eta:S^0 \rightarrow S^0$ is the Hopf map
 in $\SH(S)$.

The first step to our main theorem is the following result:
\end{num}
\begin{thm}\label{thm:heart&eta}
Consider the notations of the preceding lemma.
\begin{enumerate}
\item The adjunction of abelian categories induced by $(K,N)$
$$
\ptau_{\leq 0}(K):\pheart\SH(S) \leftrightarrows \pheart\DMt(S):N
$$
is an equivalence of categories.
\item The functor induced by $\gamma_*$
$$
\gamma_*:\pheart\DMcdh(S) \rightarrow \pheart\SH(S)
$$
is fully faithful and its essential image is
 made of the weakly orientable spectra.
\end{enumerate}
\end{thm}
\begin{proof}
The proof is based on the fact that these results
 are known when $S=\Spec(E)$ for $E$ a finite extension of $k$:
 in this case, the homotopy perverse $t$-structure
 coincides with the homotopy $t$-structure
 (Example \ref{ex:p-htp_field});
 then Point (1) follows from the explicit description
 of the heart of the homotopy $t$-structure
 (cf \cite{Mor1}) and Point (2) is the
 main result of \cite{Deg10}.

The proof will use noetherian induction
 with the help of the following lemma:
\begin{lm}
Let $S$ be an integral $k$-scheme of finite type
 with funtion field $E$.
 Let $\T$ be one of the motivic triangulated
 categories $\SH$, $\DMt$, $\DMcdh$.

Then the canonical map
$$
\pheart\T(\Spec(E)) \rightarrow \ilim_{U \subset S} \left(\pheart\T(U)\right)
$$
where the left hand side refers to the perverse homotopy
 $t$-structure with respect to $E$ as a base field,
 and the limits runs over the non empty open subscheme of $S$,
 is an equivalence of abelian categories.
\end{lm}
\begin{proof}
Note the map is well defined as for any open immersion $j$,
 $j^*$ is $t^p$-exact (Prop. \ref{prop:basic_tp-exactness}).
 The lemma now follows formally from the fact $\T$ is continuous
 (\emph{cf} \cite[Def. 4.3.2]{CD3}) and the perverse homotopy
 $t$-structure is left complete.
\end{proof}
We will prove this by induction on the dimension of $S$,
 the case of dimension $0$ being known from the above remark.
 As a first step, we can assume $S$ is integral,
 up to removing the intersection of its irreducible components.

Point (1) follows easily from this lemma and the remark
 of the beginning of the proof, by noetherian induction.

For Point (2), we first prove that $\gamma_*$ is fully faithul.
 In other words, for any object $K$ of the heart
 of $\DM(S)$, the adjunction map
$$
ad:\ptau_{\leq 0}(\gamma^*) \gamma_*(K) \rightarrow K
$$
is an isomorphism.

According to the preceding lemma and the initial remark,
 there exists an open subscheme $j:U \rightarrow S$
 such that the result is known in $\DM(U)$ for $j^*(K)$.
Let $i:Z \rightarrow X$ be the complementary closed immersion.
 According to Corollary \ref{cor:tp-glueing},
 to prove that $ad$ is an isomorphism, is suffices 
 to check that $\ptau_{\leq 0} i^*(ad)$ is an isomorphism.
 
We have the following computation:
$$
\ptau_{\leq 0} i^*\ptau_{\leq 0}(\gamma^*) \gamma_*
 \simeq \ptau_{\leq 0} (i^*\gamma^*)\gamma_*
 \simeq \ptau_{\leq 0} \gamma^*(i^*\gamma_*)
 \underset{(1)}\simeq \ptau_{\leq 0} \gamma^*(\gamma_*i^*)
 \underset{(2)}\simeq \ptau_{\leq 0} \gamma^* \gamma_* (\ptau_{\leq0}i^*)
$$
where the isomorphism (1) follows from the fact $\gamma_*$
 commutes with $j_\sharp$ and the localization property
 for $\DM$ and $\DMt$ and isomorphism (2) because $\gamma_*$
 preserves $t^p$-negative objects.
Thus, we are reduced to prove the assertion to $\ptau_{\leq0}i^*(K)$
 which follows by the induction hypothesis.

The last assertion follows similarly by induction,
 by another application
 of Corollary \ref{cor:tp-glueing}
 and the fact that condition of being weakly orientable is compatible
 with localization. 
\end{proof}
 
